Generative and deterministic deep learning models comparison for fine-scale precipitation retrievals from infrared brightness temperature

Accurate precipitation estimation at fine spatial scales is critical for hydrology, agriculture, and climate studies. Infrared brightness temperatures from geostationary satellites offer excellent temporal coverage over continental-scale domains. However, because these measurements primarily characterize cloud-top properties rather than precipitation processes near the surface, their correlation with rainfall intensity remains limited, making quantitative precipitation estimation challenging. In this study, we conduct a systematic inter-comparison of state-of-the-art deep learning models for high-resolution precipitation retrieval from Meteosat Second Generation infrared brightness temperatures over metropolitan France. These models include deterministic U-Nets, transformer-based architectures, conditional GANs, and diffusion models. We construct a curated dataset spanning 2008--2023, combining M{\'e}t{\'e}o-France radar mosaics as reference with multi-channel infrared observations, and design preprocessing and sampling strategies to address the heavy-tailed, intermittent nature of rainfall. Our results show that deterministic models provide robust mean estimates and excel in pixel-wise accuracy, but systematically underestimate extreme precipitation. In contrast, generative models better capture the full precipitation distribution, including rare and heavy rainfall events, producing more realistic spatial structures at the cost of reduced pixel-wise fidelity. These results highlight a trade-off between pixel-wise accuracy and precipitation variability, showing that generative approaches are advantageous for extreme-event detection and probabilistic applications. This work establishes a reproducible framework for evaluating infrared- based precipitation retrieval methods and provides guidance for designing models that balance precision, variability, and extreme-event representation.

==> classification__1_.tex <==
\begin{table}[htbp]
\centering
\caption{Pixel-wise rain/no-rain detection metrics for all models at a 0.2 mm/h threshold. Metrics include accuracy, precision, recall, F1 score, critical success index (CSI), and false alarm ratio (FAR). For each metric $\uparrow$ means higher is better, $\downarrow$ means lower is better and best values are shown in bold, second-best values are in italic.}
\begin{tabular}{lcccccc}
\hline
Model & Accuracy ($\uparrow$) & Precision ($\uparrow$) & Recall ($\uparrow$) & F1 ($\uparrow$) & CSI ($\uparrow$) & FAR ($\downarrow$) \\
\hline
Baseline UNet           & 0.82         & 0.64           & 0.76          & \emph{0.69} & \emph{0.53} & 0.36 \\
QuantileUNet:median & \textbf{0.84} & \textbf{0.75} & 0.62             & 0.67       & 0.51      & \textbf{0.25} \\
Multitask UNet       & \emph{0.83} & 0.66            & \emph{0.77} & \textbf{0.71} & \textbf{0.55} & 0.34 \\
DeepLabV3+          & 0.82         & 0.63         & 0.76          & 0.69         & 0.53         & 0.37 \\
SegFormer           & 0.82        & 0.62           & \textbf{0.78} & 0.69       & 0.53       & 0.38 \\
cGAN                & 0.81          & \emph{0.67}   & 0.52          & 0.59        & 0.42       & \emph{0.33} \\
Diffusion (epsilon-prediction) & 0.74 & 0.51 & 0.54 & 0.52 & 0.36 & 0.49 \\
Diffusion (image-prediction) & 0.76  & 0.56 & 0.45 & 0.50 & 0.33 & 0.44 \\
\hline
\end{tabular}
\label{tab:classification_metrics}
\end{table}
